Some results on combinators in the system TRC

We investigate the system TRC of combinatory logic that is equiconsistent with New Foundations. We prove that various unstratified combinators do not exist in TRC.

==> table.tex <==
%-*-tex-*-
% Copyright Michael J. Ferguson, INRS-Telecommunications (1985,1986)
% All rights reserved. 
\catcode`\@=11

%======= Additional active Characters ===========
% ALL ACTIVE CHARACTERS MUST BE DECLARED AND DEFINED AT THE VERY
% BEGINNING OR THERE IS A DANGER OF INCORRECT TOKENIZATION 
% ======== THESE ARE USED IN THE TABLE MACROS =========
\message{<< Additional Active Characters >>}
\catcode`\|= \active 
\def|{\ifmmode \vert\else \char`\|\fi} % effectively undoes activeness
\def\q@m{\string"}
\catcode`\"=\active \def"{\char`\"}
% update \dospecials
\toksdef\toks@@=2
\toks@{\do \"}\toks@@ =\expandafter{\dospecials}\xdef\dospecials{\the\toks@@\the\toks@}
\toks@{\do \|}\toks@@ =\expandafter{\dospecials}\xdef\dospecials{\the\toks@@\the\toks@}
%=== these are redefined inside the table macros =====


%============= Table making macros ============
% the basic format is
% \begintable
% <special definitions for this table>
% \begintableformat
%           format as in halign except it needs ## instead of #
%           in tableformat, " means strut column
%           spacing controlled by \left, \center, \right
%           can use \math or \displaymath in conjuction with spacing
% \endtableformat
% \br{<struts>} .... | .... | .... " ..... | .... \er{<stuff>}  (rows)
% \-                                                (horizontal rules)
% ....etc
% \endtable
%
% each row has format
% \br{<..>}  <item> | <item} " .... | <item> \er{<..>}
%                   \br, \er mean beginning of row, end of row
%                   in table | means rule, " means no rule in strut column
%                   \: is standard strut, | is standard vrule
%
% \tablespread {to <dimen>}  width of table
% \tr=width of rules (default .4pt)
% \midtabglue sets glue in table (default 0pt plus 1fill)
% also can set explicit hrules and vrules
% tokens (e.g. \tablespread, \tr, \midtabglue, etc.) can be set in \everytable

% these macros require that | and " be active during the entire 
% document to work correctly. ... although some definitions specifically
% set them active
\newcount\a@lignstate  \a@lignstate=0  %0 -- between lines after \cr
                                       %1 -- beginning of line in \bl
                                       %2 -- midline
                                       %3 -- endline in \el
\def\hssf{\hskip 0pt plus 1fill minus 1fill}
\def\n@ewaligndefs{\def\center##1{\hssf ##1\hssf\null}
          \def\left##1{##1\hssf\null}
          \def\right##1{\hssf ##1\null}}
\newdimen\trulesize
\let\tr=\trulesize
\trulesize = .4pt
\def\zerocenteredbox#1{\ifmmode \ifinner \setbox2 =\hbox{$#1$}\else 
                           \setbox2 =\hbox{$\displaystyle#1$}\fi
                     \else \setbox2 =\hbox{#1}\fi
      \setbox0=\hbox{\lower.5ex\hbox{$\vcenter{\box2}$}}\ht0=0pt\dp0 =0pt\box0}
\let\zb=\zerocenteredbox

%this macro creates a strut with the that is higher by #2 and deeper than #3
% than the natural size of #1 ... the sizes may be negative
\def\modifystrut#1#2#3{\setbox4=\hbox{#1}\dimen0=\ht4
             \advance \dimen0 by #2 \dimen2 = \dp4 
             \advance  \dimen2 by #3 
            \vrule width 0pt height \dimen0 depth \dimen2}
\let\mst=\modifystrut
%general math form
\def\math#1{\relax $\relax#1\relax$}
\def\displaymath #1{\relax$\displaystyle #1\relax$}


%   
\newskip\tcs  
\newtoks\tablespread
\newskip\midtabglue \midtabglue = 0pt plus 1fill
\newtoks\everytable  \everytable = {\relax}

{\catcode`\|=\active   \catcode`\" = \active
  \gdef\begintable{\vbox\bgroup \tcs=.5em % uses font in force when entering 
                  \catcode`\|=\active
                  \catcode`\"=\active
                   \def\:{\relax \vrule height 2.5ex depth .9ex width 0pt}
          \def\-{\ifcase\a@lignstate \fulltablerule{\tr}
                  \else 
                  \thrule{\tr}\fi}
          \let\t@xx =\relax % for premature expansions
          \everycr={\noalign{\global\a@lignstate=0}}
          \def\fulltablerule##1{\noalign{\hrule height
                   ##1}}
          \def\thrule##1{\omit\leaders\hrule height ##1\hfill}
          \def\center{\hskip\tcs\hss ########\hss\hskip\tcs}
          \def\left{\hskip\tcs ########\hss\hskip\tcs}
          \def\right{\hskip\tcs\hss ########\hskip\tcs}
          \def\sprule{\tvrule{2.5\tr}}
          \def|{\ifcase\a@lignstate \def\t@xx{\tvrule{\tr}}\or
                            \def\t@xx{\tvrule{\tr}}\or
                             \def\t@xx{\unskip&\tvrule{\tr}&}\else 
                             \def\t@xx{\tvrule{\tr}}\fi\t@xx}
          \def\|{\ifcase\a@lignstate \def\t@xx{\sprule}\or
                            \def\t@xx{\sprule}\or
                             \def\t@xx{\unskip&\sprule&}\else 
                              \def\t@xx{\sprule}\fi\t@xx}
          \def"{&########&} % for table format
          \def\br##1{\global\a@lignstate=1 ##1\unskip\global\a@lignstate=2&}
          \def\er##1{\global\a@lignstate=3\unskip&##1\unskip
                      \global\a@lignstate=0\cr}
          \def\tvrule##1{\hss\vrule width ##1\hss}
          \def~{\penalty\@M \hphantom{0}}
%				% changes ~ to be phantom of width .5em
          \tablespread = {}
          \the\everytable 
               }
  \gdef\begintableformat #1\endtableformat{\offinterlineskip \tabskip = 0pt
       \edef\t@blform{####\tabskip =\midtabglue &#1&####\tabskip=0pt\cr}
%						% adds rules front and back
                                  \n@ewaligndefs
                                 \def"{\ifcase\a@lignstate \def\t@xx{\relax}\or
                                          \def\t@xx{\relax}\or
                                        \def\t@xx{\unskip&&}\else 
                                        \def\t@xx{\relax}\fi\t@xx}
                                \edef\h@align{\halign \the\tablespread}
                                  \h@align\bgroup\span\t@blform}
      }% " and | are always active in INRSTEX

\def\use#1{\omit\mscount=#1 \advance\mscount by -1\multiply\mscount by2
                \loop\ifnum\mscount>1 \sp@n\repeat
                \ifnum\mscount>0 \span \else \relax \fi}
\let\sp=\span
\let\om = \omit
\def\sa#1{\setbox0=\hbox{#1}\hbox to \wd0{}}
\def\endtable{\crcr\egroup\egroup}

\catcode`\@=12

